Subtyping on Nested Polymorphic Session Types

The importance of subtyping to enable a wider range of well-typed programs is undeniable. However, the interaction between subtyping, recursion, and polymorphism is not completely understood yet. In this work, we explore subtyping in a system of nested, recursive, and polymorphic types with a coinductive interpretation, and we prove that this problem is undecidable. Our results will be broadly applicable, but to keep our study grounded in a concrete setting, we work with an extension of session types with explicit polymorphism, parametric type constructors, and nested types. We prove that subtyping is undecidable even for the fragment with only internal choices and nested unary recursive type constructors. Despite this negative result, we present a subtyping algorithm for our system and prove its soundness. We minimize the impact of the inescapable incompleteness by enabling the programmer to seed the algorithm with subtyping declarations (that are validated by the algorithm). We have implemented the proposed algorithm in Rast and it showed to be efficient in various example programs.

==> language.tex <==
\section{Formal Language Description}\label{sec:language}

\input{tab_desc}

In this section, we present the program constructs we have designed
to realize nested polymorphism which have also been integrated with the
Rast language~\cite{Das20FSCD,Das20CONCUR,Das20PPDP} to
support general-purpose programming.
The underlying base system of session types is derived from a Curry-Howard
interpretation~\cite{Caires10concur,Caires16mscs} of intuitionistic linear logic
\cite{Girard87tapsoft}. The key idea is that an intuitionistic linear sequent
$A_1 \; A_2 \; \ldots \; A_n \vdash A$
is interpreted as the interface to a process $P$. We label each of the
antecedents with a channel name $u_i$ and the succedent with channel name $z$.
The $u_i$'s are \emph{channels used by} $P$ and $z$ is the \emph{channel provided by} $P$.
\begin{mathpar}
  (u_1 : A_1) \; (u_2 : A_2) \ldots (u_n : A_n) \vdash P :: (z : C)
\end{mathpar}
The resulting judgment formally states that process $P$ provides a service of
session type $C$ along channel $z$, while using the services of session types $A_1,
\ldots, A_n$ provided along channels $u_1, \ldots, u_n$ respectively. All these
channels must be distinct. We abbreviate the antecedent of the sequent by $\Delta$.

Due to the presence of type variables, the formal typing judgment
is extended with $\vars$ and written as
\begin{center}
  \begin{minipage}{0cm}
  \begin{tabbing}
  $\vars \semi \D \vdash_\Sg P :: (u : A)$
  \end{tabbing}
  \end{minipage}
\end{center}
where $\vars$ stores the variables,
$\D$ represents the linear antecedents $u_i : A_i$, $P$ is the process
expression and $u : A$ is the linear succedent. We propose and maintain
that all free type variables in $\D, P$, and $A$ are contained in $\vars$.
Finally, $\Sigma$ is a fixed valid signature containing type and process
definitions.
%in~\autoref{subsec:base}). 
Table~\ref{tab:language} overviews the session types, their associated
process terms, their continuation (both in types and terms) and operational description.
For each type, the first line describes the provider's viewpoint, while
the second line describes the client's matching but dual viewpoint.
% Figure~\ref{fig:basic-typing} describes selected
% typing rules (ignore the premises and annotation on the turnstile
% marked in blue, introduced in Section~\ref{subsec:ergo}) leaving the complete
% set of rules to Appendix~\ref{app:formal}.

We formalize the operational semantics as a system of \emph{multiset rewriting
rules}~\cite{Cervesato09SEM}. We introduce semantic objects $\proc{c}{P}$
and $\msg{c}{M}$ which mean that process $P$ or message $M$ provide
along channel $c$.
A process configuration is a multiset of such objects, where any two
provided channels are distinct.

\subsection{Basic Session Types}\label{subsec:base}

We briefly review the structural types already existing in the Rast language,
focusing on explicit quantifier operators that we introduce.

\paragraph{\textbf{Structural Types}}
The \emph{internal choice} type constructor
$\ichoice{\ell : A_{\ell}}_{\ell \in L}$ is an $n$-ary labeled
generalization of the additive disjunction $A \ichoiceop B$.
Operationally, it requires the provider of
$u : \ichoice{\ell : A_{\ell}}_{\ell \in L}$ to send a label
label $k \in L$ on channel $u$ and continue to provide
type $A_{k}$. The corresponding process term is written as $(\esendl{u}{k} \semi P)$
where the continuation $P$ provides type $u : A_k$.
Dually, the client must branch based
on the label received on $u$ using the process term
$\ecase{u}{\ell}{Q_\ell}_{\ell \in L}$ where $Q_\ell$ is the continuation
in the $\ell$-th branch.
% \begin{mathpar}
% \infer[{\with}R]
% {\vars \semi \D \vdash \ecase{u}{\ell}{P_\ell}_{\ell \in L} ::
% (u : \echoice{\ell : A_\ell}_{\ell \in L})}
% {(\forall \ell \in L)
%  & \vars \semi \D \vdash P_\ell :: (u : A_\ell)}
% \and
% \infer[{\with}L]
% {\vars \semi \D, (u : \echoice{\ell : A_\ell}_{\ell \in L}) \vdash
% (\esendl{u}{k} \semi Q) :: (z : C)}
% {(k \in L) & \vars \semi \D, (u : A_k) \vdash Q :: (z : C)}
% \end{mathpar}
% 
% Communication is asynchronous, so that the client
% ($\esendl{c}{k} \semi Q$) sends a message $k$ along $c$ and continues as $Q$
% without waiting for it to be received. As a technical device to ensure that
% consecutive messages on a channel arrive in order, the sender also creates a
% fresh continuation channel $c'$ so that the message $k$ is actually represented
% as $(\esendl{c}{k} \semi \fwd{c}{c'})$ (read: send $k$ along $c$ and continue along
% $c'$). When the message $k$ is received along $c$, we select branch $k$ and
% also substitute the continuation channel $c'$ for $c$.
% Rules ${\with}S$ and ${\with}C$ below describe the operational behavior of the
% provider and client respectively $\fresh{c'}$.
% % \vspace{-0.2em}
% \begin{tabbing}
% $({\with}S) : \m{proc}(d, c.k \semi Q) \;\mapsto\; \m{msg}(c', c.k \semi \fwd{c'}{c}),
% \m{proc}(d, Q[c'/c])$ \\
% $({\with}C):$ \= $\m{proc}(c, \m{case}\;c\;(\ell \Rightarrow Q_\ell)_{\ell \in L}),
% \m{msg}(c', c.k \semi \fwd{c'}{c})
% \;\mapsto\; \m{proc}(c', Q_k[c'/c])$
% \end{tabbing}
% 
The \emph{external choice} constructor $\echoice{\ell : A_{\ell}}_{\ell \in L}$
generalizes additive conjunction and is the \emph{dual} of internal
choice reversing the role of the provider and client. Thus, the provider
branches on the label $k \in L$ sent by the client.
% \begin{mathpar}
%   \infer[{\oplus}R]
%     {\vars \semi \D \vdash (\esendl{u}{k} \semi P) :: (u : \ichoice{\ell : A_\ell}_{\ell \in L})}
%     {(k \in L) & \vars \semi \D \vdash P :: (u : A_k)}
%   \and
%   \infer[{\oplus}L]
%     {\vars \semi \D, (u : \ichoice{\ell : A_\ell}_{\ell \in L}) \vdash
%     \ecase{u}{\ell}{Q_\ell}_{\ell \in L} :: (z : C)}
%     {(\forall \ell \in L) &
%       \vars \semi \D, (u : A_\ell) \vdash Q_\ell :: (z : C)}
% \end{mathpar}
% This dual constructor reverses the role of the provider and client.
% The provider $(\esendl{u}{k} \semi P)$ of $u : \ichoice{\ell : A_\ell}_{\ell \in L}$
% sends the label $k$ along $u$ and continues to provide $u : A_k$.
% Correspondingly, the client branches on the label received using channel
% $u : A_\ell$ in branch $\ell$ with process term $Q_\ell$.
% The rules of operational semantics (${\oplus}S, {\oplus}C$) are the dual
% of ${\with}S$ and ${\with}C$ and omitted for brevity.

The \emph{tensor} operator prescribes that the provider of
$u : A_2 \tensor B$
sends a channel, say $z$ with type $A_1$, subtype of $A_2$ in a context of variance $\cov$, 
and continues to provide type $B$. The
corresponding process term is $\esendch{u}{z} \semi P$ where $P$ is
the continuation.  Correspondingly, its client must receive a channel on $u$
using the term $\erecvch{u}{w} \semi Q$, binding it to variable $w$
and continuing to execute $Q$.
 \begin{mathpar}
   \infer[{\tensor}R]
     {\vars \semi \D, (w : A_1) \vdash (\esendch{u}{w} \semi P) :: (u : A_2 \tensor B)}
     {\vars \semi \D \vdash P :: (u : B)
     \and 
     \vars \semi \cdot \vdash A_1 \leq A_2 \ofv \cov}
%   \and
%   \infer[{\tensor}L]
%     {\vars \semi \D, (u : A \tensor B) \vdash (\erecvch{u}{w} \semi Q) :: (z : C)}
%     {\vars \semi \D, (w : A), (u : B) \vdash Q :: (z : C)}
 \end{mathpar}
% Operationally, the provider $(\esendch{c}{d} \semi P)$ sends the
% channel $d$ and the continuation channel $c'$ along $c$ as a message and
% continues with executing $P$. The client receives the channel $d$ and continuation
% channel $c'$ and substitutes $d$ for $u$ and $c'$ for $c$.
% \begin{tabbing}
% $({\tensor}S) : \m{proc}(c, \m{send}\; c\; d \semi P) \;\mapsto\; $\=
% $\m{proc}(c', P[c'/c]),
% \m{msg}(c, \m{send}\; c\; d \semi \fwd{c}{c'})$ \\
% $({\tensor}C) : $ \= $\m{msg}(c, \m{send}\; c\; d \semi \fwd{c}{c'}),
% \m{proc}(e, u \leftarrow \m{recv}\; c \semi Q)
% \;\mapsto\; \m{proc}(e, Q[c', d/c, u])$
% \end{tabbing}

The dual operator, \emph{lolli}, allows the provider to receive a
channel of type $A_2$ and continue to provide type $B$. The client
of $A_2 \lolli B$, on the other hand, sends the channel of type $A_1$,
subtype of $A_2$,
and continues to use $B$ using dual process terms as $\tensor$.
 \begin{mathpar}
%   \infer[{\lolli}R]
%     {\vars \semi \D \vdash (\erecvch{u}{w} \semi P) :: (u : A \lolli B)}
%     {\vars \semi \D, (w : A) \vdash P :: (u : B)}
%   \and
   \infer[{\lolli}L]
     {\vars \semi \D, (u : A_2 \lolli B), (w : A_1) \vdash (\esendch{u}{w} \semi Q) :: (z : C)}
     {\vars \semi \D, (u : B) \vdash Q :: (z : C) \and 
     \vars \semi \cdot \vdash A_1 \leq A_2 \ofv \cov}
 \end{mathpar}

% \paragraph{\textbf{Termination}}

The type $\one$
indicates \emph{termination} requiring that the provider of $u : \one$
send a \emph{close} message, formally written as $\eclose{u}$
followed by terminating the communication. Correspondingly,
the client of $u : \one$ uses the term $\ewait{u} \semi Q$
to wait for $u$ to terminate before continuing with executing $Q$.
% Linearity enforces that the provider does not use any channels.
% \begin{mathpar}
%   \infer[{\one}R]
%     {\vars \semi \cdot \vdash (\eclose{u}) :: (u : \one)}
%     {q = 0}
%   \and
%   \infer[{\one}L]
%     {\vars \semi \D, (u : \one) \vdash (\ewait{u} \semi Q) :: (z : C)}
%     {\vars \semi \D \vdash Q :: (z : C)}
% \end{mathpar}
% Operationally, the provider waits for the closing message, which
% has no continuation channel since the provider terminates.
% \begin{tabbing}
% $({\one}S) : \m{proc}(c, \m{close}\; c) \;\mapsto\; \m{msg}(c, \m{close}\; c)$ \\
% $({\one}C) : $ \= $\m{msg}(c, \m{close}\; c),
% \m{proc}(d, \m{wait}\; c \semi Q) \;\mapsto\; \m{proc}(d, Q)$
% \end{tabbing}

% \paragraph{\textbf{Forwarding}}
A forwarding process $\fwd{u}{w}$ identifies the channels $u$ and $w$ so that any
further communication along either $u$ or $w$ will be along the unified channel.
 \begin{mathpar}
   \infer[\m{id}]
     {\vars \semi w : A \vdash (\fwd{u}{w}) :: (u : B)}
     {\vars \semi \cdot \vdash A \leq B \ofv \cov}
 \end{mathpar}
% Operationally, a process $\fwd{c}{d}$ \emph{forwards} any message M
% that arrives on $d$ to $c$ and vice-versa. Since channels are used
% linearly, the forwarding process can then terminate, ensuring proper
% renaming, as exemplified in the rules below.
% \begin{tabbing}
% $(\m{id}^+C) : $ \= $\m{msg}(d', M),
% \m{proc}(c, \fwd{c}{d}) \;\mapsto\; \m{msg}(c, M[c/d])$ \\
% $(\m{id}^-C) : $ \= $\m{proc}(c, \fwd{c}{d}),
% \m{msg}(e, M(c)) \;\mapsto\; \m{msg}(e, M(c)[d/c])$
% \end{tabbing}
% We write $M(c)$ to indicate that $c$ must occur in message $M$ ensuring that $M$ is the
% sole client of $c$.

% Operationally, the intuition is realized by forwarding: a process $\fwd{c}{d}$
% forwards any message $M$ that arrives along $d$ to $c$ and vice-versa.
% Because channels are used linearly the forwarding process can then terminate,
% making sure to apply the proper renaming.
% The corresponding rules of operational
% semantics are $\m{id}^+C$ and $\m{id}^-C$ in Figure~\ref{fig:basic-opsem}.

The remaining formal rules of the type system and operational semantics for the above
structural session types are skipped for brevity and available in the  
literature on Rast~\cite{Das20PPDP,DasDMP21}.

\paragraph{\textbf{Process Definitions}}
Process definitions have the form
$\D \vdash f\indv{\alpha} = P :: (u : A)$ where $f$ is the name of the
process and $P$ its definition, with $\D$ being the channels used
by $f$ and $u : A$ being the offered channel. In addition, $\overline{\alpha}$
is a sequence of type variables that $\D$, $P$ and $A$ can refer to.
All definitions are collected in the fixed global signature $\Sg$.
For a \emph{valid signature}, we
require that $\overline{\alpha} \semi \D \vdash P :: (u : A)$
for every definition, thereby allowing
definitions to be mutually recursive. A new instance of a defined
process $f$ can be spawned with the expression
$\ecut{u}{f \indv{A}}{\overline{w}}{Q}$ where $\overline{w}$ is a
sequence of channels whose types are supertypes of 
the antecedents $\D$,
and $\overline{A}$ is a sequence of types matching the type
variables $\overline{\alpha}$.
The newly spawned process will use all variables in
$\overline{w}$ and provide $u$ to the continuation $Q$.
% \vspace{-0.5em}
 \begin{mathpar}
   % \vspace{-0.5em}
   \inferrule*[right=$\m{def}$]
   {\overline{w':B'} \vdash f \indv{\alpha} = P_f :: (u' : B) \in \Sg \quad
   \vars \semi \cdot \vdash \D' \leq \overline{(w:B')}[\overline{A}/\overline{\alpha}] \ofv \cov \quad
   \vars \semi \D, (u : B[\overline{A}/\overline{\alpha}]) \vdash Q :: (z : C)}
   {\vars \semi \D, \D' \vdash (\ecut{u}{f \indv{A}}{\overline{w}}{Q}) :: (z : C)}
 \end{mathpar}
 The declaration of $f$ is looked up in the signature $\Sg$ (first premise),
 and $\overline{A}$ is substituted for $\overline{\alpha}$ while
 matching the types in $\D'$ and $\overline{w}$ (second premise). Similarly,
 the freshly created channel $u$ has type $A$ from the signature
 with $\overline{A}$ substituted for $\overline{\alpha}$.
 The corresponding semantic rule can be found in the literature~\cite{Das20PPDP,DasDMP21}.
% The corresponding semantics rule also performs a similar substitution
% $\fresh{a}$.
% \begin{tabbing}
% $(\m{def}C) : $ \= $\m{proc}(c, \ecut{u}{f \indv{A}}{\overline{d}}{Q}) \; \mapsto \;
% \m{proc}(a, P_f[a/u, \overline{d}/\overline{w'}, \overline{A}/\overline{\alpha}]), \;
%    \m{proc}(c, Q[a/u])$
% \end{tabbing}
% where $\overline{w' : B'} \vdash f = P_f :: (u' : B) \in \Sg$.

Sometimes a process invocation is a tail call,
written without a continuation as $\procdef{f \indv{A}}{\overline{w}}{u}$. This is a
short-hand for $\procdef{f \indv{A}}{\overline{w}}{u'} \semi \fwd{u}{u'}$ for a fresh
variable $u'$, that is, we create a fresh channel
and immediately identify it with $u$.

% \paragraph{\textbf{Type Definitions}}
% Although type definitions are often used in session types, 
% the usage of type definitions with type parameters, makes 
% this a distinguishing feature of \polymorphicsessiontypes.

% Session types can be defined
% recursively, departing from a strict Curry-Howard interpretation of
% linear logic, analogous to the way pure ML or Haskell depart from
% a pure interpretation of intuitionistic logic. 
% %%
% Taking advantage of type constructors, \polymorphicsessiontypes\ 
% further enable \emph{polymorphic recursion} on the definition of types.
% Recall that a type definition for a type name $V$ is of the form 
% $V \indv{\alpha} = A$, where $\overline{\alpha}$ denotes a sequence of
% type variables that $A$ can refer to.
% The signature $\Sg$ contains all type definitions,
% that are possibly mutually recursive.
% For a well-formed signature, we require $A$ to be
% contractive.
% %%
% Our type definitions are \emph{equirecursive} so we can
% silently replace indexed type names $V \indv{B}$ by $A
% [\overline{B}/\overline{\alpha}]$ during type checking,
% and no explicit rules for recursive types are needed.

% All types in a signature $\Sg$ must be \emph{valid}, formally written
% as $\vars \vdash \valid{A}$ requiring that all free type variables in
% $A$ are contained in $\vars$.

\paragraph{\textbf{Explicit Quantifiers}}
We introduce two \emph{novel dual type constructors}, $\texists{x} A$
and $\tforall{x} A$ to exchange types between processes.
The existential type $\texists{x}A$ requires the provider
to send a valid type $B$ and  continue to provide $A[B/x]$. The
validity of $B$ is ensured by a pre-pass that we perform 
checking that all types are valid. The
term used to send a type is $(\esendch{u}{[B]} \semi P)$ where $P$
is the continuation. Dually, the client receives a type using the
expression $(\erecvch{u}{[x]} \semi Q)$, binds it to variable
$x$, and then continues to execute $Q$ using the session type $A$
which possibly contains the free variable $x$. The corresponding
typing rules are
\begin{mathpar}
  \infer[{\exists}R]
    {\vars \semi \D \vdash (\esendch{u}{[B]} \semi P) :: (u : \texists{x}A)}
    { %\vars\semi \cdot \vdash B \ofv \xi \and
    \vars \semi \D \vdash P :: (u : A[B/x])}
  \and
  \infer[{\exists}L]
  	{\vars \semi \D, (u : \texists{x}A ) \vdash (\erecvch{u}{[x]} \semi Q) :: (z : C)}
    { \vars \semi \D, (u : A) \vdash Q :: (z : C)}
\end{mathpar}

Operationally, the provider $(\esendch{u}{[B]} \semi P)$ sends the
type $B$ and the continuation channel $c'$ along $c$ and
continues executing $P$. The client receives the type $B$ and continuation
channel $c'$ and substitutes $B$ for $x$ and $c'$ for $c$ in Q.
\begin{tabbing}
$({\exists}S) \;\, \m{proc}(c, \m{send}\; c\; [B] \semi P) \;\mapsto\; $\=
$\m{proc}(c', P[c'/c]),
\m{msg}(c, \m{send}\; c\; [B] \semi \fwd{c}{c'})$ \\
$({\exists}C) $ \= $\m{msg}(c, \m{send}\; c\; [B] {\semi} \fwd{c}{c'}),
\m{proc}(e, [x] \leftarrow \m{recv}\; c {\semi} Q)
\mapsto \m{proc}(e, Q[c', B/c, x])$
\end{tabbing}

Dually, a provider with a universal typed session $\tforall{x}A$ 
receives an arbitrary type, binds it to $x$, and proceeds to provide
session prescribed by type $A$, possibly referring $x$.
On the other hand, the client sends a valid type $B$ and 
continues with session $A[B/x]$.
The judgment $\vars \vdash \valid{B}$ denotes that free variables
in $B$ are bound in $\vars$.
\vspace{-0.5em}
\begin{mathpar}
  \vspace{-0.5em}
  \infer[{\forall}R]
  	{\vars \semi \D \vdash (\erecvch{u}{[x]} \semi P) :: (u : \tforall{x}A)}
    {\vars \semi \D \vdash P :: (u : A)}
  \and
  \infer[{\forall}L]
  	{\vars \semi \D, (u : \tforall{x}A ) \vdash (\esendch{u}{[B]} \semi Q) :: (z : C)}
    {  \vars\semi \cdot \vdash B \ofv \xi \and
    \vars \semi \D, (u : A [B/x]) \vdash Q :: (z : C)}
\end{mathpar}

\subsection{Type Safety}\label{subsec:soundness}
The extension of session types with nested polymorphism
is proved type safe by the standard theorems of
\emph{preservation} and \emph{progress}, also known as
\emph{session fidelity} and \emph{deadlock freedom}.
At runtime, a program is represented using a multiset of semantic
objects denoting processes and messages defined as a \emph{configuration}.
\begin{center}
  \begin{minipage}{0cm}
  \begin{tabbing}
  $\config \; ::= \; \cdot \mid \config, \config' \mid \proc{c}{P} \mid \msg{c}{M}$
  \end{tabbing}
  \end{minipage}
\end{center}
We say that $\proc{c}{P}$ (or $\msg{c}{M}$) provide channel $c$.
We stipulate that no two distinct semantic objects in a configuration
provide the same channel.

\paragraph{\textbf{Type Preservation}}
The key to preservation is defining the rules to
\emph{type a configuration}.
We define a well-typed configuration
using the judgment $\D_1 \Vdash_{\Sg} \config :: \D_2$
denoting that configuration $\config$ uses channels $\D_1$
and provides channels $\D_2$. A configuration is always
typed w.r.t. a valid signature $\Sg$.
Since the signature $\Sg$ is fixed, we elide it from
the presentation.

\begin{figure}[t]
  \begin{mathpar}
  \infer[\m{emp}]
  {\D \Vdash (\cdot) :: \D}
  {}
  \and
  \infer[\m{comp}]
  {\D_1 \Vdash (\config_1, \config_2) :: \D_3}
  {\D_1 \Vdash \config_1 :: \D_2 \and
  \D_2 \Vdash \config_2 :: \D_3}
  \and
  \infer[\m{proc}]
  {\D \Vdash \proc{u}{P} :: (u:A)}
  {\cdot \semi \D \vdash P :: (u : A)}
  \and
  \infer[\m{msg}]
  {\D \Vdash \msg{u}{M} :: (u:A)}
  {\cdot\semi \D \vdash M :: (u : A)}
  \end{mathpar}
  \vspace{-1em}
  \caption{Typing rules for a configuration}
  \vspace{-1em}
  \label{fig:config_typing}
\end{figure}

The rules for typing a configuration are defined in
Figure~\ref{fig:config_typing}.
The $\m{emp}$ rule states that an empty configuration
does not consume any channels provides all channels it uses.
The $\m{comp}$
rule composes two configurations $\config_1$ and $\config_2$;
$\config_1$ provides channels $\D_2$ while $\config_2$ uses
channels $\D_2$. The rule $\m{proc}$ creates a singleton configuration
out of a process. Since configurations are runtime objects,
they do not refer to any free variables and $\vars$ is empty.
The $\m{msg}$ rule is analogous.

\paragraph{\textbf{Global Progress}}
To state progress, we need to define a \emph{poised
process}~\cite{Pfenning15fossacs}.  A process $\proc{c}{P}$ is
poised if it is trying to receive a message on $c$. Dually, a message
$\msg{c}{M}$ is poised if it is sending along $c$. A configuration
is poised if every message or process in the configuration is
poised. Intuitively, this represents that the
configuration is trying to communicate \emph{externally} along
one of the channels it uses or provides.
\begin{theorem}[Type Safety]\label{thm:type_safety}
  For a well-typed configuration $\D_1 \Vdash_{\Sg} \config :: \D_2$,
  \begin{enumerate}
    \item[(i)] (Preservation) If $\config \step \config'$, then
    $\D_1 \Vdash_{\Sg} \config' :: \D_2$

    \item[(ii)] (Progress) Either $\config$ is poised, or $\config \step
    \config'$. 
  \end{enumerate}
\end{theorem}

\begin{proof}
  Preservation is proved by case analysis on the rules of
  operational semantics. First, we invert the derivation of
  the current configuration $\config$ and use the premises to
  assemble a new derivation for $\config'$.
  Progress is proved by induction on the right-to-left typing of $\config$
  so that either $\config$ is empty (and therefore poised) or $\config =
  (\dc, \proc{c}{P})$ or $\config = (\dc, \msg{c}{M})$. By the induction
  hypothesis, either $\dc \step \dc'$ or $\dc$ is poised.
  In the former case, $\config$ takes a step (since $\dc$ does).
  In the latter case, we analyze the cases for $P$ and $M$,
  applying multiple steps of inversion to show that in each case either
  $\config$ can take a step or is poised.
\end{proof}



==> tab_desc.tex <==
\begin{table*}[t]
  \centering
  \small
  \begin{tabular}{l l l l l}
  \textbf{Type} & \textbf{Cont.} & \textbf{Process Term} & \textbf{Cont.} & \multicolumn{1}{c}{\textbf{Description}} \\
%   \textbf{(current)} & & \textbf{(current)} & & \\
  \toprule
  $c : \ichoice{\ell : A_\ell}_{\ell \in L}$ & $c : A_k$ & $\esendl{c}{k} \semi P$
  & $P$ & send label $k$ on $c$ \\
  & & $\ecase{c}{\ell}{Q_\ell}_{\ell \in L}$ & $Q_k$ & receive label $k$ on $c$ \\
  \addlinespace
  $c : \echoice{\ell : A_\ell}_{\ell \in L}$ & $c : A_k$ & $\ecase{c}{\ell}{P_\ell}_{\ell \in L}$
  & $P_k$ & receive label $k$ on $c$ \\
  & & $\esendl{c}{k} \semi Q$ & $Q$ & send label $k$ on $c$ \\
  \addlinespace
  $c : A \tensor B$ & $c : B$ & $\esendch{c}{z} \semi P$
  & $P$ & send channel $z : A$ on $c$ \\
  & & $\erecvch{c}{w} \semi Q_w$ & $Q_w[z/w]$ & receive channel $z : A$ on $c$ \\
  \addlinespace
  $c : A \lolli B$ & $c : B$ & $\erecvch{c}{w} \semi P_w$
  & $P_w[z/w]$ & receive channel $z : A$ on $c$ \\
  & & $\esendch{c}{z} \semi Q$ & $Q$ & send channel $z : A$ on $c$ \\
  \addlinespace
  $c : \texists{x}A $ & $c : A[B/x]$ & $\esendch{c}{[B]} \semi P$
  & $P$ & send type $B$ on $c$ \\
  & & $\erecvch{c}{[x]} \semi Q_{x}$ & $Q_{x}[B/{x}]$ & receive type $B$ on $c$ \\
  \addlinespace
  $c : \tforall{x}A $ & $c : A$ & $\erecvch{c}{[x]} \semi P_{x}$
  & $P_{x}[B/x]$ & receive type $B$ on $c$ \\
  & & $\esendch{c}{[B]} \semi Q$ & $Q$ & send type $B$ on $c$ \\
  \addlinespace
  $c : \one$ & --- & $\eclose{c}$
  & --- & send $\mi{close}$ on $c$ \\
  & & $\ewait{c} \semi Q$ & $Q$ & receive $\mi{close}$ on $c$ \\
  \bottomrule
  \end{tabular}
  \caption{Session types with operational description}
  \label{tab:language}
  \vspace{-2em}
  \end{table*}
  

==> tab_syntax.tex <==
\begin{table}
  \centering
  \begin{tabular}{l l l}
  \textbf{Abstract Type\quad} & \textbf{Concrete Type\quad} & \textbf{Concrete Syntax} \\
  \toprule
  $\texists{x} A$ & \verb|?[x]. A| & \verb|send x [B]| \\
  $\tforall{x} A$ & \verb|![x]. A| & \verb|[B] <- recv x| \\
%  $V\indv{x}$ & \verb|V[x1]...[xk]| \\
  \bottomrule
  \end{tabular}
  \caption{Abstract and Corresponding Concrete Syntax}
  \label{tab:syntax}
  \vspace{-1.5em}
\end{table}
  
